Toward Next Generation Open Radio Access Network--What O-RAN Can and Cannot Do!

The open radio access network (O-RAN) describes an industry-driven open architecture and interfaces for building next generation RANs with artificial intelligence (AI) controllers. We circulated a survey among researchers, developers, and practitioners to gather their perspectives on O-RAN as a framework for 6G wireless research and development (R&D). The majority responded in favor of O-RAN and identified R&D of interest to them. Motivated by these responses, this paper identifies the limitations of the current O-RAN specifications and the technologies for overcoming them. We recognize end-to-end security, deterministic latency, physical layer real-time control, and testing of AI-based RAN control applications as the critical features to enable and discuss R&D opportunities for extending the architectural capabilities of O-RAN as a platform for 6G wireless.

==> include/contribution.tex <==
\textcolor{blue}{Extend AI control through the MAC and PHY, from our proposal}
\textcolor{blue}{Describe the architectural changes. and changes proposed in santos.et al (2021) about RANaaS and its security implications}
\textcolor{blue}{Also, explore the integration of transfer learning and architectural changes required for it}

==> include/directions.tex <==
\textcolor{blue}{Can be implicitly described in the previous sections or summarized here}


==> include/resources.tex <==
In this section, we outline the available resources that enable the realization of an open, interoperable and AI driven RAN. %system. 
We first introduce the O-RAN specifications which lays the design foundations and then go on to describe some of the tools and testbeds which have incorporated these principles.

\subsection{Standardization}
\subsubsection{O-RAN Alliance}
%\textcolor{blue}{How organized, who participates, what is standardized}
The O-RAN Alliance was formed by merging the C-RAN Alliance %~\cite{} 
and the xRAN forum%~\cite{}
and leads the open RAN movement that aims to extend the current RAN standards to facilitate open, intelligent, virtualized and fully interoperable next generation RANs. 
Many of its members are also members of the 3GPP. 

 %The O-RAN standards 
Its study items cover the overall O-RAN architecture and is divided into main nine technical work groups (WG):
%The WGs are: 
\begin{itemize}
    \item WG1: Use cases and overall architecture,
    \item WG2: %the %non-real-time RAN intelligent controller
    Non-RT RIC and A1 interface,
    \item WG3: %the %Near-real-time 
    Near-RT RIC and E2 interface,
    \item WG4: Open fronthaul interfaces, 
    \item WG5: Open F1/W1/E1/X2/Xn interface,
    \item WG6: Cloudification and orchestration,
    \item WG7: White-box hardware, 
    \item WG8: stack reference design, and
    \item WG9: open X-haul transport.
\end{itemize}
In addition, there are four O-RAN focus groups (FG) that handle items %topics 
related to the overall mechanism of O-RAN:
\begin{itemize}
    \item FG1: standard development,
    \item FG2: test \& integration,
    \item FG3: open source, and
    \item FG4: security. 
\end{itemize}

Figure~\ref{fig:ORANStnds} illustrates the WGs and FGs defined by the O-RAN Alliance along with the main contributions of each group. The working groups meet regularly and updated specifications are published and made accessible to the community every three months.


% %\subsubsection{Telecom Infrastructure Project (TIP)}
% \hl{Did TIP take off or is it phasing out? If still popular, let's keep it here.} TIP was intially formed by Facebook with a focus on enabling access for all and is currently headed by Vodafone~\cite{}. Unlike the O-RAN Alliance, which mainly concerns itself with an open and interoperable RAN, TIP has many project groups that span a diverse set of wireless communication systems. The project groups are categorized into three main groups which include many sub-groups within them:
% \begin{itemize}
%     \item Product project groups : Focuses on identification of areas in need of innovation. It is divided into three network areas that collectively make up an end-to-end network viz,
%     \begin{itemize}
%         \item Access Projects : RAN Initiatives, Open Cellular and OpenRAN - TIP 
%     \end{itemize}
    
%     \item Solution Project groups
%     \item Software Project groups
% \end{itemize}
% While the O-RAN Alliance heavily focuses on 4G and 5G, TIP 
% \begin{itemize}
%      \item WG1: Use Cases and Overall Architecture Workgroup
%      \item WG2: The Non-real-time RAN Intelligent Controller and A1 Interface Workgroup
%      \item WG3: The Near-real-time RIC and E2 Interface Workgroup
%      \item WG4: The Open Fronthaul Interfaces Workgroup
%      \item WG5: The Open F1/W1/E1/X2/Xn Interface Workgroup
%      \item WG9: Open X-haul Transport Workgroup
%      \item TIFG: Test & Integration Focus Group 
     
%  \end{itemize}

 
%O-RAN Alliance described in Work Grope 1 (WG1) specifications different use cases that leverage the O-RAN architecture and demonstrate its unique benefits to optimize a RAN function and update policies based on performance measurement. some of these used cases deploy one of the aforementioned ML deployment scenario in the O-RAN architecture. 


\subsection{Software} \label{software}
\subsubsection{O-RAN Software Community}
The O-RAN Alliance together with the Linux Foundation officially launched the O-RAN software community (OSC) in April 2019 for the realization of O-RAN components and systems via open-source software. The first code release of the OSC was the Amber release in December 2019. It was been developed by 60 developers across 10 companies and provides initial implementation of the near-RT RIC, O1 interface, and the protocol stack. In June 2020, the Bronze release was the result of 80 contributors from 15 companies. The Bronze contributions focused on the development of the O-DU, O-CU, O1 and A1 interfaces. The Cherry release was presented in December 2020 involving of 60 developers from 10 companies. The Cherry release advances the O1 and A1 interfaces implementations and introduces the E2 interface with end-to-end integration and focus on the SMO components for management and self-organization. The %most recent release, called 
Dawn became available in July 2021 and provides evolved A1, E2, and O1 interfaces with more advanced xApps for near-RT RIC, non-RT RIC use cases and O-DU specifications. A new R1 interface between rapps and SMO/non-RT RIC services was also introduced. Figure.~\ref{fig:ORANStnds} shows the O-RAN software development timeline. % starting from the launching up to the expected E release.

\subsubsection{ONF SD-RAN}
The Open Networking Foundation's software-defined RAN (SD-RAN) project engages in a parallel open source development effort that aims to integrate the 3GPP compliant RAN with the O-RAN RIC and its interfaces along with a few exemplar xApps. The first release of SD-RAN came out in Januray 2021 with support for a near-real time RIC based on ONF's $\mu$ONOS and Aether(VIM) platforms. Open Air Interface 5G~\cite{} enhanced with O-RAN compliant protocols and interfaces is employed to undertake O-DU and O-CU functionalities.  An SDK, portable across different near-RT RIC platforms for the xApp development has also been released. This means that the SDK can also be used in OSC's system. SD-RAN's vision is to expand the E2 interface to allow for scheduler control and implement use cases related to network slicing, handover and load balancing. 

While the SD-RAN uses OAI-5G and potentially provides hardware compatibility, it is designed as a production grade software directed at companies developing intelligent xApps. Therefore SD-RAN's offerings are protected by a member only software license The software framework developed by the OSC implements the control stack and does not support hardware enabled RAN systems yet. Simulated environments such as the O-DU/O-CU code base ~\cite{} and the Viavi RAN simulator~\cite{} serve as options to test and validate the working of the O-RAN system but fall short in terms of measuring the performance in a realistic wireless environment. This served as an inspiration for various independent working groups to develop a hardware compliant Open RAN ecosystem to fully enable design, analysis and testing of solutions in a real-world setting. 
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/ORAN/ORAN_SW.pdf}
% %\vspace{-70 pt}
% \caption{O-RAN software development timeline.}
% \label{fig:ORANSW}
% \vspace{-3mm}
% \end{figure}


\subsection{Testbeds}
%\begin{itemize}[leftmargin=+9.4pt]
%\item
  

The Platforms for Advanced Wireless Research (PAWR) is a public-private partnership program that supports the develops and maintains five large-scale wireless testbeds, four in realistic outdoor environments and one large-scale programmable RF emulator. It is a National Science Foundation (NSF) initiative. Several PAWR platforms currently work on O-RAN implementations, discussed in continuation.

%\textbf{POWDER:} 
The Platform for Open Wireless Data-driven Experimental Research (POWDER)~\cite{breen2021powder} is a city scale, remotely accessible, end-to-end software defined platform that supports mobile and wireless research. It is deployed in Salt Lake City, Utah. %POWDER has so far deployed over a dozen fixed and approximately fifty mobile programmable radio nodes over an area of 14 square kilometers, covering a variety of distinct environments such as urban, moderate density and residential environments. Experiments over a range of heterogeneous wireless technologies including massive MIMO, 5G, RAN are supported. 
The testbed is equipped with cutting edge software-defined radios (SDRs), commercial off-the-shelf (COTS) equipment and computing resources at both the edge and cloud to support low latency interactions. An experimenter %also allows an experimenter to
can instantiate a series of profiles---a set of experiment environments for popular 4G/5G software stacks, such as srsRAN and OpenAirInterface%(OAI)
, and the Open Network Automation Platform (ONAP) for network control and orchestration. An O-RAN capable profile %with  capabilities was added. It
implements the communication between the near-real time RIC and the RAN node simulated by srsRAN. An xApp featuring basic RAN slicing was also developed to demonstrate how a RAN node can be controlled by the near-RT RIC based on inputs from a \hl{What is this and is it too much detail?}REST server~\cite{Johnson21NexRAN}. 
%to   Some of the "sister" projects of POWDER 

%\textbf{COSMOS}: 
The Cloud-Enhanced Open Software Defined Mobile Wireless Testbed for City-Scale Deployment (COSMOS)~\cite{raychaudhuri2020challenge} is based in New York City. % covering 1 square mile of densely populated neighborhood in West Harlem, New York. 
The focus of COSMOS is on ultra high bandwidth and low-latency communications by employing mmWave and dynamic optical switching technologies and coupling it with edge computing.
COSMOS includes the Open-Access Research Testbed for Next-Generation Wireless Networks (ORBIT)~\cite{} which is compatible with open RAN solutions and served as the Open Test and Integration Center to demonstrate multi-vendor interoperability during the O-RAN plugfest~\cite{}.

% AERPAW (focusing on aerial communication).... 

%\textbf{COLOSSEUM:}
The Colosseum testbed is %one of the world's most powerful full stack
an SDR-based wireless network emulator~\cite{} %based in Burlington, MA at 
that was developed by DARPA and is now maintained by Northeastern University. % Innovation campus. 
%The testbed is a specialized datacenter with up to 900TB of storage, 171 servers, 320 FPGAs and a total of 25.6 GHz of instantaneous bandwidth. 
It includes 256 programmable SDRs (USRP X310s) out of which 128 are dedicated to a massive channel emulator. % (MCHEM) which can emulate almost any real world scenario such as open fields, dense urban cities, deserts, shopping malls etc. %The rest of the 128 nodes are available to experimenters. The MCHEM can emulate fading, multipath for upto 256x256 independently customizable channels. Additionally, the testbed supports cellular networks (4G, 5G), IoT networks, edge computing and cloud based RAN research. 
Several applications are preconfigured by Colosseum and can be instantiated by experimenters in the form of %ready to use 
LXC containers, which can also be customized by users. %The containers can also be customizable by users to implement their own radio codes. The platform also allows implementation and testing of machine learning algorithms for various wireless techniques including spectrum sharing, dynamic spectrum access (DSA) and optimized routing. ML algorithms can be tested by collecting RF data at a rate of 52 TB/s from heterogeneous wireless networks. \hl{Can we elaborate more on O-RAN on Colosseum, and shorten the rest?} 
Recently, open-source RAN solutions were made available with the inclusion of the %O-RAN 
near-RT RIC interfaced with srsLTE~\cite{bonati2020intelligence}. %Colosseum was initially used in DARPA's Spectrum Collaboration Challenge (SC2) until the finals in 2019 and will be available to researchers through NSFs PAWR program henceforth. The testbed is accessible as a cloud based platform where users can reserve resources and schedule experiments manually or configure it as a batch job. 

% {latest PAWR testbed ...}
%\item 
%{\textbf{COLLOSEUM Testbed:}}

%\textcolor{blue}{Briefly comparison of these resources and their capabilities}
 
\subsection{OAIC}
%\textbf{Open Artificial Intelligence Cellular (OAIC):} 
%\hl{Vuk will revise} 
Open Artificial Intelligence Cellular (OAIC) is a large-scale community research infrastructure project that focuses on developing a 6G research framework. It implements and extends the O-RAN framework and interfaces, develops AI controllers, and an AI controllers/O-RAN network testing framework for use with SDR testbeds. It closes the gap between testbed hardware and 5G protocol software development and deployment to enable AI-controlled 5G and 6G research. %and maintenance and community SDR research testbed, such as the PAWR platforms. 
%... a mobile community research testbed infrastructure based in \hl{.....} 
OAIC aims to supplement open SDR platforms and community testbeds with AI-enhanced, O-RAN compliant wireless network functions and controllers to enable research on next generation RANs and advance the %O-RAN 
specifications. 
OAIC also develop the tools and procedures for designing and testing AI-enhanced wireless networks in controlled and production-like environments. %and It is a platform that enables designing and testing AI-driven 6G RAN use cases. The testbed consists of multiple programmable SDRs (B210s and N300s) and servers capable of simulating LTE/5G systems. Recently, the testbed included O-RAN capabalities where the communication between the near-real time RIC and the RAN node, using srsLTE 
%was established. 
Using servers, COTS SDR hardware, and exclusively open-source software, the OAIC team implemented the interfaces between the near-RT RIC and the software-defined LTE base station (srsRAN) and developed a resource allocation xApp %has been developed where the xApp 
which makes decisions on the number of physical resource blocks (PRBs) that have to be allocated to SDR UEs transmitting on both uplink and downlink in a controlled %n SDR LTE 
testbed environment. 
%\end{itemize}



==> include/services.tex <==
\textcolor{purple}{O-RAN is a highly disruptive technology that opens up the RAN to multiple vendors, virtualizes the RAN software, and several other capabilities and usecases detailed in this section. This will bring several benefits to mobile network operators -- reduce the costs, multi-vendor ecosystem, quick time to market for new services, enable highly dynamic services, and greater level of innovation in RAN domain.}


%\textcolor{blue}{Features: disaggregation-standard interfaces-multi-vendor support, intelligence, different timescales that are supported, openness, software, \\

%Introduce those, if not already, and explain what these features enable...}

%\input{Tables/TechnologiesTable}
\input{Tables/ORANusecasesTable}


\subsection{Dynamic Disaggregation %, Functional Splits, 
and Multi-Vendor Support %\hl{combine with C?--there is a lot of repetition and may be difficult to split cleanly}
}
\textcolor{purple}{The discussion under this subsection is pretty long, and possibly not needed. Can we not simply say the following? O-RAN supports 3GPP RAN disaggregation - CU, DU, and RU and standard interfaces among them. Specifically, O-RAN adopt ..... FS Option 2... for .... and Option 7.2x for .... Furthermore, as presented in Section III, O-RAN supports additional standard interfaces such as, E2, O1, A1. Because of this support for RAN disaggregation and open interfaces, O-RAN will support the multi-vendor ecosystem enabling  more competition and vibrant supplier ecosystem which will bring down the RAN cost significantly.}
% The 3GPP introduced the FS in Release 15 %for 5G
% to allow splitting the baseband %unit BBU 
% functionalities into the %{Centralized Unit}
% CU---responsible for non-RT higher layer 2 (L2) and L3 functions---and the DU%{Distributed Unit}
% ---responsible for RT L2 %scheduling 
% and L1 functions. 
\textcolor{blue}{3GPP introduced the FS in Release 15 to allow splitting the base station 
functionalities into the CU and the DU, implementing the higher and lower layers of the RAN protocol stack, respectively. %%---responsible for %non-RT 
%%higher layer protocol %2 (L2) and L3
%%functions---and the DU---responsible for %RT L2 and L1 
%%the lower layer functions.
3GPP Technical Specifications (TS) 38.801 define many different split options---Options 1-8 (Fig.~\ref{fig:fs}a) plus suboptions---that allow balancing between more centralized or more distributed signal processing. %, which has implications on the midhaul or F1 interface requirements in terms of bandwidth and latency. For example, a split option that implements a lightweight DU, e.g. a portion of the PHY layer (Option 7), puts more stress on the F1 interface than a DU that implements the entire PHY and MAC (Option 4) or more.
} 

\begin{figure}[ht]
	   \centering
	   \includegraphics[width=0.49\textwidth]{figures/fs.pdf}
\vspace{-6mm}
\caption{3GPP FS options (a) and the O-RAN FSs and interfaces between the O-CU, O-DU, and O-RU (b).}
\label{fig:fs}
\end{figure}

The introduction of flexible FSs promotes the disaggregation, softwarization, and virtualization of the RAN functionalities and enables operators to shape network features and use cases as per the application requirements and deployment scenarios. 
Depending on the bandwidth and latency requirements, it is possible to deploy both the CU and DU functions %either 
centrally or at the edge, close to 
the RU. Even if the components are collocated, different %the actual 
protocol stack splits can be implemented to best meet %might be different based on 
the service/application requirements. %This also allows 
\textcolor{blue}{Many} CU/DU functions can be implemented as virtual \textcolor{blue}{network %software
functions (VNFs)} and be deployed in any RAN tier on commercial off-the shelf hardware\textcolor{blue}{, as has been demonstrated for software radio implementations of a 4G or 5G RAN~\cite{5GWF18,AlyCommMag22}}. Load management, RT performance optimization, and maintenance of various QoS requirements for different applications %like gaming and voice
can thus be handled through multiple instances of the CU and the DU that share the same physical resources, thereby reducing cost and increasing network performance. 
In practice, these %splits 
are implemented as containers managed by a hypervisor\textcolor{blue}{, or virtual machine monitor,} to ensure scalabiltiy, diverse network support, and interoperability. 

Although %\hl{The} 
3GPP defines many different split options across protocol layers, % different levels, 
the \hl{vendors} have %\textcolor{blue}{closed standards}
\textcolor{blue}{proprietary implementations and interfaces}
\sout{lock-in} which has lead to single vendor solutions. %in practice implies that the software which implements the CU and the DU is limited to the chosen vendor. 
The openness of the O-RAN  architecture and interfaces enables cellular operators to employ unique strengths of each vendor for a delicate application or service and facilitates RAN function sharing. % purposes. 
\textcolor{blue}{It is envisaged that} the near-RT RIC and non-RT RIC \textcolor{blue}{will be able to support} different vendors' CUs and DUs to efficiently use the resources for different use cases. 
%%Unlike traditional RAN architectures, O-RAN envisions the use of standardized interfaces to make network sharing practical, %a key feature 
%for reducing cost and s known as . 
%Here, due to the openness and virtualization of RAN components
where physical infrastructure operators can %share their wireless infrastructure and 
host %logical 
CU and DU implementations as virtual network function (VNFs) from multiple vendors~\cite{5GWF18}.

\textcolor{blue}{%\hl{The O-RAN Alliance/software community initially/currently} 
O-RAN adopted %the 3GPP 
FS Option 2 for the F1 interface between the O-DU and O-CU (higher-layer split--HLS), and %\hl{the O-RAN specific} 
Option 7-2x for implementing the fronthaul, the interface between the O-DU and O-RU (lower-layer split--LLS) \cite{REF?}. Figure~\ref{fig:fs} illustrates this with reference to the FS options defined by %the
3GPP.
O-RAN employs a modified version of the common public radio interface (CPRI), the enhanced CPRI (eCPRI), for the fronthaul specifications. %The eCPRI relies on split option 7-2x—the low PHY-high PHY split—, where the higher PHY layer functions of the O-DU are separated from the lower PHY layer functions of the O-RU. 
} %The 7-2x FS implements part of the PHY in the O-RU and the rest in the O-DU.
%The number of options for such splits increases as we move from the CU to the RU. %/PHY layer. 
 %\hl{O-RAN very brief here:} %\hl{Is the remaining information needed and are you talking about the LLS or HLS and about 3GPP or O-RAN? Does 3GPP also have two splits, LLS and HLS, or is the RU integrated into the DU in 3GPP?} \textcolor{red}{The LLS and HLS is used in 3GPP and adopted for O-RAN, and it is based on which unit support which protocol stack function. CU provides support for the higher layers of the protocol stack such as SDAP, PDCP, and RRC; while the DU provides support for the lower layers of the protocol stack such as RLC, MAC, and physical layer.} %Taking into consideration these factors,
The O-RAN Alliance has adopted FS \textcolor{blue}{7-2x} because it provides the best support for 4G/5G systems, whereas %and indicated 
FS 8 works best for 2G/3G systems. Other application specific splits include FS 6 for small cells and FS 7 for dense urban areas %where several RUs are deployed to increase capacity and 
where the fronthaul %\hl{capacity can be provided} 
performance is critical~\textcolor{blue}{\cite{ORANFH}}. 
\hl{Why do we talk about FS x and FS y, should we not say LLS x and LLS y? A FS can refer to LLS and HLS, right?}
\textcolor{blue}{The O-RAN fronthaul interface as well as the F1 interface are open and, if implemented consistently, will allow connecting O-CUs, O-DUs, and O-RUs from different software developers and hardware vendors.}
%\hl{Should we comment on FS 7-2x here since we use it in several figures?--we do later}
%This split is cost effective and lets operators share gains through a distributed approach while maintaining the lowest processing utilizations on the DU and RU. 


% \subsubsection{The O-RAN Selected Split 7-2x}
% \begin{itemize}
%     \item Interface simplicity:
%     \item Transport Bandwidth Scalability:
%     \item Beamforming Support:
%     \item Interoperability:
%     \item Advanced receivers and inter-cell coordination:
%     \item Lower O-RU complexity:
%     \item Future proofness:
%     \item Interface and functions symmetry:
% \end{itemize}

% \subsection{Implementation Options of O-RAN}

% \begin{itemize}
%     \item Shared Cell:
%     \item Near-RT RIC:
% \end{itemize}




%\subsubsection{O-RAN Timescale Analysis}
\subsection{Support for Different Timescales} %Non and Near-Real-Time %Timescale 
%Support}
%\textcolor{blue}{This subsection can come before the previous. I suggest introducing the 3 AI control loops in this section, unless they fit better in Section II, for instance.} %\textcolor{blue}{Do we need a subsection or could it be a simple paragraph under Integration of AI/ML?}
% \Vijay{Also, this time scale is not just about AI.. It's about RAN control loops like, it is okay to do slicing in minutes or hours, whereas scheduling needs to be done in milliseconds. Beamforming may be required to be done in milliseconds or seconds depending upon the mobility of users. See the control loops table in Northeastern paper.}
One of the main requirements for meeting the heterogeneous 5G services\textcolor{blue}{, such as interference management, resource allocation and scheduling, security, and traffic offloading,} %with the O-RAN architecture 
is being able to perform RAN operations at the appropriate timescales. In 5G, the network may respond with resource changes %on the 
at sub-millisecond time granularity. %order. % of $1$ ms. %~\cite{5G_book}. %, whereas 6G systems are expected to operate respond to an order of magnitude faster. To enable this, 
The O-RAN Alliance defines the closed-loop control of the RAN by enabling the RIC to operate at different timescales: 
\begin{itemize}
    \item \textbf{The non-RT control loop} %- The control loop 
    operates at a timescale of at least 1 s through the A1 and O1 interfaces. Examples include instantiation and orchestration of network slices, resource allocation at the infrastructure level and data driven RAN policy guidance to xApps in the near-RT RIC. Such decisions can be taken at frequencies spanning seconds, hours, or even days.
    \item \textbf{The near-RT control loop} %- This control loop 
    operates on a timescale between 10 ms and 1 s through the E2 interface. The xApps hosted on the near-RT RIC %serve \hl{lighter detection purposes} and
    leverage user session data and MAC and PHY layer data to optimize the %user 
    Quality of Experience (QoE) by controlling time sensitive services, such as resource scheduling, beamforming, load balancing, and handover. % processes. 
    % \item real time control loop - This control loop takes care of the operations of a cellular network at the sub-10 ms or sub-ms timescale. These sub-ms tasks are currently not a part of O-RAN implementation since it requires high level computation and RU level standardization.
\end{itemize}
%This will require AI output with very low latency.
Combining the fast processing at the near-RT RIC with the larger timescale analysis at the non-RT RIC %and SMO 
is a unique capability of the O-RAN architecture. \textcolor{blue}{Table~\ref{tab:ORANuse} shows some of the RAN operations that can be implemented via utilizing the different timescales properties of the O-RAN enabled by the non-RT and near-RT control loops.}% that aims to provide O-RAN with a small response time. 
% To explain, xApps can be embedded within the near-RT RIC for a lighter detection purpose, while the AI analytic algorithms can be applied at the non-RT RIC or externally to perform more complicated processing and then transfer the obtained policy to near-RT RIC over A1 interface.

\subsection{\textcolor{red}{Open Interfaces and Multi-Vendor Support} \hl{Remove this section because of Reviewer 5, Comment 6 and because all of it is already covered in III and IV.A}}
%\hl{Outline how interfaces are different from 3GPP interfcaes. Outline RAN sharing. }

\textcolor{red}{The openness of the O-RAN  architecture and interfaces enables cellular operators to employ unique strengths of each vendor for a delicate application or service and facilitates RAN function sharing.} % purposes. 
\textcolor{red}{It is envisaged that the near-RT RIC and non-RT RIC will be able to support different vendors' CUs and DUs to efficiently use the resources for different use cases. }


\textcolor{red}{3GPP networks implement %typically utilize 
the common public radio interface (CPRI) protocol for exchanging data between the remote radio units and the baseband unit. The CPRI is based on the lower layer split 8, where the RF unit is detached from the baseband processing. % PHY layer. %\hl{However, the openness, virtualization, RAN disaggregation, and intelligence features of O-RAN cannot be achieved through the CPRI or split 8}. \textcolor{blue}{Can you explain why?} Therefore, t
The needs for more flexibility, reliability with higher transmission rates have motivated the O-RAN to employ a modified version of the CPRI, which is known as the enhanced CPRI (eCPRI) for the fronthaul specifications. The eCPRI relies on split option 7-2x---the low PHY-high PHY split---, where the higher PHY layer functions of the O-DU are separated from the lower PHY layer functions of the O-RU. Figure~\ref{fig:Compare} illustrates the difference between the CPRI and eCPRI protocols from the FS perspective. }

\textcolor{red}{Additionally, to support the disaggregation strategy, 3GPP also introduces the F1 interface that connects the CU to the DUs and the E1 interface to enable coordination between the control and user planes at the CU. % units. 
The O-RAN Alliance %parallelly
defines additional complementary interfaces, such as the E2 interface which coordinates the control of the RAN through the RIC, and the A1 interface, which communicates with the SMO. 
These interfaces implement standardized data driven workflows and facilitate the operation of control loops between the RIC and the RAN functions at different timescales. For example, the E2 interface supports near-RT control of the RAN (order of 10 ms - 1 s), whereas the O1 interface assists with the non-RT control. Unlike traditional RAN architectures, O-RAN envisions the use of standardized interfaces that make network sharing practical, %a key feature 
%for reducing cost and s known as . 
%Here, due to the openness and virtualization of RAN components
where physical infrastructure operators can share their wireless infrastructure and host %logical 
CU and DU implementations as virtual network function (VNFs)~\cite{5GWF18}. A remote E2 interface can monitor and control the DU while a remote O1 interface can be used to communicate the desired  VNF configurations.}




\subsection{\sout{Integration of AI} \textcolor{purple}{AI Integration and xApps/rApps}}

The O-RAN architecture %design 
provides the capability of simultaneously collecting %the %required 
application %information 
and radio environment information to perform intelligent decisions based on the retrieved information using AI models. Such capability is not supported by the \hl{conventional and emerging}\textcolor{red}{``conventional and emerging'' needs to be changed or explained as per reviewer 1.10 comment} base stations, but is supported by design of the O-RAN specifications. \textcolor{blue}{ Where the recent advances in intelligent automation of 3GPP networks is provided by the network data analytics function (NWDAF) that is limited to support 5G core network functions only.} %gNB/eNB of 5G and 4G cellular networks. 

\textcolor{blue}{The non-RT RIC is a controller of the SMO %platform for 
that 
provides policy management, AI management, and data enrichment services to the underlying RAN nodes. The AI management services %of the non-RT RIC 
includes the transfer of the trained model to the near-RT RIC in the RAN and the periodic or triggered updates of the AI model. The data enrichment capability of the non-RT RIC %focusing on
delivers the required information to the near-RT RIC, which performs data analytic and management functions\sout{ to draw conclusions, make predictions, and drive informed decisions}.}

The variability of key performance indicators (KPIs) and QoS levels of %the provided 
5G use cases %and applications 
along with the existing operation and maintenance functions of cellular networks enable %that are able only on 
optimizing the cellular performance parameters per cell. % not individually.
The O-RAN technology, on the other hand, enables performance enhancements per UE from the collected information, such as long-term traffic, coverage, and observed interference. %, an then performing it via the near-RT RIC to the gNB for execution.
Integrating the resource management %scheduling process of different 
 %from the core network %'s QoS mechanism 
in the near-RT RIC %function module 
is beneficial for reducing the burden on the core network as well as reducing the data transfer and time overhead of forwarding and processing data between the RAN and the core network. This %e newly introduced intelligence at the RAN
%can  time in transmission process, which overall 
improves the overall efficiency and latency of the system.   


% \begin{itemize}
%      \item \textbf{QoE Optimization}: this use case automates the configuration and controlling of RAN parameters to improve the QoE of the user by utilizing the intelligent and open interface of the O-RAN architecture. The limited radio resources are utilized in a way that the  UE's use specific applications that requires critical KPI e.g. Cloud VR assign sufficing radio resources to meet these KPI and improve there QoE. The ML solution for this case consists of training model at the Non-RT RIC to obtain QoE related models such as Application Classification Model, QoE Prediction Model, QoE policy Model and Available BW Prediction Model. The offlkine model will use the training data data in table~\ref{tab:ORANuse} which provided by the E2 node over the O1 interface. After the training phase, the QoE related ML model will be deployed in Near- RT RIC to assist in the QoE Optimization function. The Near- RT RIC
%  \end{itemize}



\textcolor{blue}{The near-RT RIC can host third-party control applications, i.e. xApps.} 
AI is expected to improve several functionalities that software-defined RANs will be responsible for. Among those are load balancing, resource utilization, fault detection, and security. Table~\ref{tab:ORANuse} provides details about \sout{select} \textcolor{blue}{various} use cases \textcolor{blue}{for different applications and network functions }that are defined by The O-RAN Alliance~\textcolor{blue}{\cite{WG1}}. It describes several opportunities for AI \textcolor{blue}{as xApps in the near-RT RIC or rApps in the non-RT RIC} for practical cellular networks implementing the O-RAN interfaces. %SDN controllers have the greatest level of access to the system making them a high value target to attackers. 

\textcolor{purple}{Furthermore, besides collecting and training AI models for xApps in near-RT RIC, the non-RT RIC can itself host AI-driven third-party control applications, i.e., rApps, such as, AI-based orchestration of network slices and data-driven policy management to improve the automation and management of RAN resources and near-RT RIC xApps.}

%\subsection{Control of Different Network Layers}
%\textcolor{blue}{Would it make sense to emphasize here how ORAN provides opportunities to control different layers of the RAN (MAC, RLC, RRC, ....) to match it with Section V.D below}



% One of the application for the AI in the MAC layer is the dynamic spectrum access. The spectrum access is being a big challenge for the next generation wireless network where a massive number of diverse devices try to access the spectrum at the same time. The traditional model based spectrum access can't have a good performance for real time spectrum access in this case due to the heterogeneous of the  devices. Learning based random access and dynamic spectrum access has the potential to realize smart or intelligent spectrum management to support spectrum access of a massive number of devices, especially when there is a large amounts of data that can be leveraged to train an AI model and predict the characteristic of the spectrum. The result of the prediction models can be used to make a decision to use the spectrum or not in order to maximize a reward function. This rewards function could be the spectrum utilization, power consumption, load balancing and such network performance. A one case where the AI based dynamic spectrum access model can be used is when there are two class of users for the spectrum, primary users(PU) and secondary users (SU). PUs are users who are currently registered on the network and possess a high priority to access the access the spectrum  where SUs are users who are not registered but want to access the network and can only use the spectrum when there is an idle space. The reward function here id the spectrum efficiency and minimum interference to the PUs. AI-enabled learning models (e.g., SVM and DNN) can be used to  detect the spectrum working status by categorizing each feature vector (spectrum) into either of the two classes, namely, the “spectrum idle” and “spectrum busy”, and adaptively update the leaning models based on dynamic environments. Then, the SUs can use the prediction results of the AI model in order to make a decision to use the spectrum in this time or not. 



% \begin{figure}[t]
 %    \centering
  %   \includegraphics[width=0.48\textwidth]{figures/RIC.png}
   %  \caption{O-RAN use case RRM based Qos}
    % \label{fig:RIC}
     %\vspace{-3mm}
 %\end{figure}

% \subsection{Beamforming}
% O-RAN supports the following beamforming methods
% \begin{itemize}
%     \item Predefined-beam beamforming:
%     \item Weight-based dynamic beamforming:
%     \item Attribute-based dynamic beamforming:
%     \item Channel-information-based beamforming:
% \end{itemize}

==> include/testbeds.tex <==
\subsection{O-RAN Software Community}
The O-RAN Alliance~\cite{openranalliance} has teamed up with the Linux foundation and has established the O-RAN Software Community (OSC)~\cite{oransoftwarecommunity} to develop open source software compliant with O-RAN specifications~\cite{}. Led by a consortium of major operators and vendors featuring the likes of AT&T, Nokia, Intel, Radisys, 3 releases viz., “amber”, “bronze”, “cherry” have been published. 

% The RIC deployment follows the cloud-based architecture and is implemented on COTS hardware. The near-RT RIC installed on VM has containers for each of its components. The docker containers need to be loaded with the respective images built from the provided source code. Once that is done, the built images need to be hosted on a server from where they can be pulled. Another simpler approach would be to directly pull the docker images from the nexus server hosted by OSC. 

\subsection{ONAP Implementation}
ONAP is an NFV framework developed as a project of the Linux Foundation and major telecom operators such as AT&T, China Mobile, Vodafone, etc. ONAP is deployed in several commercial cellular networks, and vendors like Ericsson, Nokia, Huawei and ZTE, among others, provide ONAP support and integration in their products. Therefore, ONAP represents one of the most advanced software-based solutions for commercial cellular networks, actively maintained and developed to meet production-level quality standards and satisfy new emerging requirements.
ONAP handles the design, creation, and life cycle management of a variety of network services. Network operators can use ONAP to orchestrate the physical and virtual infrastructure
deployed in their networks, in a vendor-agnostic way. In addition to common NFV orchestrator functionalities (e.g., automated policy-driven management of the virtualization infrastructure and of the network services), ONAP provides a design framework to model network applications and services as well as a framework for data analytics to monitor the services for healing and scaling. Additionally, ONAP provides a number of reference designs, i.e., blueprints. 
% These can be used to deploy the ONAP architecture, depicted at a highlevel in Figure 12, in specific markets or for specialized use cases (i.e., 5G networks or Voice over LTE deployments). They
have been tested in combination with their typical hardware configurations.
The main components of 

\subsection{PAWR Testbeds} 
The Platform for Open Wireless Data-driven Experimental Research (POWDER)~\cite{breen2021powder} is a city scale, remotely accessible, end-to-end software defined platform that supports mobile and wireless research currently deployed in Salt Lake City, Utah. Developed as a part of the National Science Foundation (NSF) Platforms for Advanced Wireless Research Programs (PAWR). POWDER has deployed over a dozen fixed and approximately fifty mobile programmable radio nodes over an area of 14sq.km. covering a variety of distinct environments such as urban, moderate density and residential environments. Experiments over a range of heterogeneous wireless technologies including massive MIMO, 5G, RAN is supported. The testbed is equipped with cutting edge SDRs, COTS equipment and computing resources at both the edge and cloud to support low latency interactions. The platform also allows an experimenter to instantiate a series of "profiles" - set of experiment environments for popular 4G/5G software stacks such as srsRAN, OpenAirInterface, ONAP for network control and orchestration. Recently a profile with O-RAN capabilities was added  to   Some of the "sister" projects of POWDER include  COSMOS~\cite{raychaudhuri2020challenge} (focusing on mmWave technology) and AERPAW (focusing on aerial communication). COSMOS includes the Open-Access Research Testbed
for Next-Generation Wireless Networks (ORBIT) ~\cite{} which is compatible with open RAN solutions and served as the Open Test and Integration Center to demonstrate multi-vendor interoperability during the O-RAN plugfest~\cite{}.

\subsection{COLLOSEUM Testbed}
\textcolor{blue}{Comparison of these resources and their capabilities}

